Can Contrastive Learning Refine Embeddings

Recent advancements in contrastive learning have revolutionized self-supervised representation learning and achieved state-of-the-art performance on benchmark tasks. While most existing methods focus on applying contrastive learning to input data modalities such as images, natural language sentences, or networks, they overlook the potential of utilizing outputs from previously trained encoders. In this paper, we introduce SIMSKIP, a novel contrastive learning framework that specifically refines input embeddings for downstream tasks. Unlike traditional unsupervised learning approaches, SIMSKIP takes advantage of the output embeddings of encoder models as its input. Through theoretical analysis, we provide evidence that applying SIMSKIP does not result in larger upper bounds on downstream task errors than those of the original embeddings, which serve as SIMSKIP's input. Experimental results on various open datasets demonstrate that the embeddings produced by SIMSKIP improve performance on downstream tasks.

==> cikm/001_introduction.tex <==

Embedding symbolic data such as text, graphs, and multi-relational data has become a key approach in machine learning and AI ~\cite{nickel2017poincare}. The learned embeddings can be utilized in various applications. 
Despite the progress in representation learning, learning effective embeddings remains a challenging problem. Deep learning models often require a large amount of labeled training data, which can be costly and limit their applicability. These are known as supervised learning tasks. Additionally, the learned embeddings often perform well on one task but not on others. To address this issue, contrastive learning has been proposed as a solution that can learn good representations with only a limited amount of labeled data.

Contrastive learning has the advantage of being able to learn representations without label information, thus saving a significant amount of human effort and resources that would have been used for data labeling. The fundamental idea of contrastive learning is to bring together an anchor and a "positive" sample in the embedding space while pushing apart the anchor from many "negative" samples ~\cite{simCLR}. Although the concept is simple, recent research has shown that contrastive learning methods can achieve comparable results to supervised methods ~\cite{NEURIPS2020_d89a66c7,robinson2021contrastive,you2021graph}.



Given the success of contrastive learning, a logical question to ask is whether using the output of another embedding model as input to contrastive learning can further refine the embedding space and make it perform better for downstream tasks. This is the question we aim to answer in this paper. We propose a new approach, \myModel, that takes the output embedding of another model as input and applies skip connection based contrastive learning on it. Our proposed method aims to fine-tune the input embedding space, making it more robust for downstream tasks. 
We theoretically prove that after applying \myModel\ on the input embedding space, for a downstream task, its error upper bound with the new learned fine-tuned embedding will not be larger than that with the original input embedding.
We conduct extensive experiments on various datasets and downstream tasks to evaluate the performance of our proposed approach and compare it with other state-of-the-art methods. The results show that the proposed \myModel\ can refine the input embedding space and achieve better performance on downstream tasks.

In summary, the main contributions of this paper are threefold: ({\bf Problem Definition}) to the best of our knowledge, we are the first to propose and investigate the use of contrastive learning to refine the embedding space.
({\bf Algorithm}) We propose a skip-connection-based contrastive learning model, \myModel, and theoretically prove that it will not increase the error upper bound of downstream tasks. ({\bf Empirical Evaluations}) We conducted extensive experiments on several real-world datasets and various downstream tasks. The results of our experiments demonstrate the effectiveness of \myModel.


%The remainder of the paper is organized as follows. Section ~\ref{problem-definition} defines the problem and introduces the notation used throughout the paper. Section ~\ref{method} describes the overall framework of the proposed algorithm and its technical details.
%Experimental results are presented in Section ~\ref{experiment}, and related work is discussed in Section ~\ref{related_work}. The paper concludes in Section ~\ref{conclusion}.




==> cikm/002_problem_definition.tex <==



In this paper, we use $D$ denoting the input dataset.
$\mathcal{X}$ denotes the original embedding space.
$T$ denotes the downstream task.
$x$ is the original embedding.
$f$ denotes the new embedding function after applying our proposed contrastive learning method \myModel.


\subsection{Contrastive Learning}

Contrastive learning aims to learn effective representations by pulling semantically similar samples together and pushing dissimilar samples apart ~\cite{gao2021simcse}.
In an unsupervised setting, constructing positive and negative pairs from unlabeld data is a critical aspect of contrastive learning.
Various data augmentation schemes are used to generate similar or positive samples (e.g., commonly used methods in visual representations include cropping, flipping, distortion, and rotation ~\cite{simCLR}).
After building positive and negative pairs, a neural network-based encoder $f()$ is used to extract representation vectors from augmented data examples. The output representation vectors of the encoder are used as the final embedding of the input data.

To learn an effective embedding space, the output of $f()$ should be easily separable by a simpler neural network, $p()$, called a projector.
$p()$ maps representations to the space where the contrastive loss is applied. A commonly used projector is a single-layer MLP, which is simple to implement.
Typically, during training, a random sample of $N$ examples is taken as a minibatch.
$2N$ data-augmented examples are derived from the minibatch.
Two augmentations from the same data point are treated as the positive pair, while the remaining $2N - 2$ data examples are treated as negative examples.
The commonly used contrastive learning loss is

\begin{equation}
l_{i,j} = - \textrm{log} \frac{\textrm{exp}(\textrm{sim}(z_i, z_j) / \tau)}{ \sum_{k=1}^{2N} \mathbf{I}_{  k \neq i } \textrm{exp}(\textrm{sim}(z_i, z_k) / \tau) }
\end{equation}
where $\tau$ is the temperature, $\textrm{sim}$ is a similarity function such as the cosine similarity, $z_i (= p(f(x_i))$ is the output of the projector ~\cite{simCLR}.

\subsection{Problem Statement}

In this paper, we focus on investigating whether contrastive learning can refine the embeddings.
Given an input dataset $D = \{d_i\}_{1}^{N}$ and an arbitrary embedding function $h()$, its output embedding is denoted as $\mathcal{X}$, where $x_i \in \mathcal{X}$ is the embedding of data point $d_i$, and $x_i = h(d_i)$.
Our goal is to design a new embedding function $f()$ such that $f(h(d_i))$ can perform better or not worse than $h(d_i)$,
which means 
given an arbitrary downstream task $\mathrm{T}$,
the performance of $\mathrm{T}$ on the embedding space generated by $f()$ should be not worse than that generated by $h()$.
Formally, the problem can be defined as

\begin{pro-stat}{Learning refined embedding with contrastive learning: }

	\textbf{Given:} (1) the embedding $\mathcal{X}$, (2) an embedding function $f()$; 
	
	\textbf{Output:} the new embedding $f(\mathcal{X})$
\end{pro-stat}

==> cikm/003_method.tex <==



In this section, we will delve into the specifics of using \myModel\ to fine-tune pre-existing embeddings.



\subsection{Contrastive Learning Limitation}


The architecture of contrastive learning ensures that augmentations of the same data point are close to each other in the embedding space. However, this alone does not guarantee that the learned embeddings are suitable for downstream tasks. 
As shown in Figure ~\ref{problem_of_existing_method}, assuming we have 8 input embedding points that belong to two different classes, red and blue. When adding Gaussian noise to the original embedding points to create their augmentations, the augmented positive points are represented by the circles around the points on the left side of the figure.
Assuming we have two different contrastive learning encoders, $f_1$ and $f_2$, they will map all augmentations of the same data point to the same embedding point in the contrastive embedding space.
If the two augmentations are denoted as $x_{i1}$ and $x_{i2}$, $\textrm{sim}(f_1(x_{i1}), f_1(x_{i2}))$ will be 1. The same for $f_2$. 
Since all the other augmentation examples are treated as negative examples, it is clear that the contrastive loss of $f_1$ will be the same as that of $f_2$.

Even though the contrastive loss of $f_1$ and $f_2$ are the same, the performance of the downstream classification task may differ between the two embedding spaces.
For example, $f_1$ separates the red and blue points into distinct clusters, making it easy for the downstream classification task to accurately classify them. However, in the embedding space created by $f_2$, the red and blue points are mixed together, resulting in poor performance for the downstream classification task.
If we use the output embedding of another model as input data, $\bar{\mathcal{X}}$, we would still encounter the same problem. 

\begin{figure}
    \centering
    \includegraphics[width=0.35\textwidth]{img/problem_of_existing_method2.png}
    \vspace{-1\baselineskip}
    \caption{The problem of existing unsupervised contrastive learning. %The image is from ~\protect\cite{xxxxxfasdfasfs}.
    }
    \vspace{-1\baselineskip}
    \label{problem_of_existing_method}
\end{figure}

\subsection{\myModel\ Details}

\begin{figure*}
    \centering
    \includegraphics[width=0.99\textwidth]{img/skip_connection5.png}
    \vspace{-1\baselineskip}
    \caption{The Skip Connection. The picture of Adapter is from ~\cite{houlsby2019parameterefficient}.}
    \label{skip_connection}
    \vspace{-1\baselineskip}
\end{figure*}

To address this problem, we introduce skip connection contrastive learning. This method is similar in principle to ResNet ~\cite{resnet} as illustrated in Figure ~\ref{skip_connection}. The idea behind skip connections is that a specific network architecture defines a class of functions $\mathcal{F}$ that it can represent.
Assuming $f^{'}$ is the optimal function we aim to find, if it is within $\mathcal{F}$, we are in good shape. However, it is often the case that it is not. Therefore, our goal is to find the best approximation of $f^{'}$ within $\mathcal{F}$.

A naive way to achieve this is to increase the depth and width of the neural network. By adding more layers and neurons, the network can represent a new class of functions $\mathcal{F}'$, which is more expressive than $\mathcal{F}$.
In general, we expect that $f_{\mathcal{F}'}$ would be better than $f_\mathcal{F}$, as a more expressive function class should be able to capture more complex patterns in the data. 
However, 
%if $\mathcal{F}'$ is not a subset of $\mathcal{F}$, 
this may not be the case. 
In fact, increasing the depth and width of the network can lead to 
a worse $f_{\mathcal{F}'}$, as illustrated by Figure ~\ref{skip_connection} (b). 
In this example, even though $\mathcal{F}_6$ is larger than $\mathcal{F}_3$, its optimal approximation is farther from the optimal function $f'$.

To solve this problem, Kaiming et al in ~\cite{resnet} proposes to use skip-connection to avoid the aforementioned issue from the non-nested function classes. 
The idea of skip-connection is that it can create nested function classes where $\mathcal{F}_1 \subseteq ... \subseteq \mathcal{F}_6$ as shown on the right of Figure ~\ref{skip_connection} (b).
Because the larger function classes contain the smaller ones, it can guarantee that increasing them strictly increases the expressive power of the network. 
For deep neural networks, 
if we can train the newly-added layer into an identity function $f(x) = x$, the new model will be as effective as the original model. 
As the new model may get a better solution to fit the training dataset, the added layer might make it easier to reduce training errors.


Building on the idea of incorporating skip connections, we propose a model named \myModel\ that utilizes contrastive learning to refine embedding based on the original input embedding. The architecture of \myModel\ is illustrated in Figure ~\ref{skip_connection} (c).
\myModel\ follows the traditional contrastive learning framework and consists of two components: a skip connection based encoder and a projector. The data encoder is a multi-layer neural network with skip connections between each two layers. The projector is a Multi-layer Perceptron (MLP) with one hidden layer, represented as $W_2 \sigma (W_1 x)$, where $\sigma$ is a ReLU non-linearity.
By incorporating skip connections, the expressive power of the network (contrastive learning encoder) is increased. Therefore, the new learned embedding should perform at least as well as the original embedding in downstream tasks.

\subsection{Data Augmentation}\label{data_aug}
Data augmentation is commonly used in contrastive learning to generate positive samples for a given data point. However, when the input to the contrastive model is the output embedding of another model, traditional data augmentation methods are not applicable. 

Inspired by ~\cite{xxxxxfasdfasfs}, in this paper, we use two types of data augmentation which are masking and adding Gaussian noise. 

\noindent{\bf A - Random Masking.}  Random masking is applied to the input embedding. Specifically, given an input embedding $x_i \in R^{d}$, a random vector $M \in \{0, 1\}^d$ is created where 0 indicates that the element will be masked and 1 indicates no change. The number of 0s in $M$ is drawn from a Bernoulli distribution $B(1 - \alpha)$, where $\alpha$ is a hyperparameter. The output after applying random masking is $x_i \circ M$, where $\circ$ represents element-wise multiplication.

\noindent{\bf B - Gaussian Noise.} When adding Gaussian noise to the input embedding $x_i \in R^{d}$, a random vector $\epsilon \sim N(0, \textbf{I} )$ is first sampled from a multi-variable Gaussian distribution, where $\epsilon \in R^{d}$ and each element in $\epsilon$ is drawn from a Gaussian distribution with 0 mean and unit variance. The output after adding the Gaussian noise is $x_i + \delta \circ \epsilon$, where $\delta$ is a hyperparameter.







\subsection{Theoretical Proof}
Let $\mathcal{X}$ denote the set of all possible data points,
traditionally, a simple multi-layer neural network (MLP) can be denoted as 
$f_1(x) = \Pi_{l=1}^L W^l x$
where $W^l$ is the model parameter of the $l$th layer. A neural network with skip connection for very two layers can be denoted as 
$f_2(x) = \Pi_{l=1}^{L/2} (W^{2l}W^{2l-1} + \mathrm{I}) x$. 
Note that $f_1$ and $f_2$ have the same amount of layers.
Suppose we have a neural network $f_I(x) = \Pi_{l=1}^L \mathrm{I} x$ where $\mathrm{I}$ is the identity matrix.
In this way, we can write the network with skip connection as
$f_2(x) = f_I + f_1(x)$.


Contrastive learning assumes access to similar data in the form of pairs ($x$, $x^+$) that come from a distribution $\mathcal{X}$ as well as $k$ i.i.d. negative samples $x_1^-, x_2^-, ..., x_k^-$. 
Learning is done over $\mathcal{F}$, a class of representation functions $f: \mathcal{X} \longrightarrow R^d$, $f$ is the contrastive encoder. 
The quality of $f$ (contrastive encoder) is evaluated by its performance on a multi-class classification task $\mathrm{T} \in \mathcal{T}$ using linear classification. 
A multi-class classifier for $\mathrm{T} \in \mathcal{T}$ is a function $g$ (we abuse the notation here)  whose output coordinates are indexed by the classes $c$ in task $\mathrm{T} \in \mathcal{T}$.
In SimCLR ~\cite{simCLR}, $g(x) = w f(x)$. 
The two losses considered in ~\cite{bound} are the standard hinge loss $l(v) = \textrm{max}\{0; 1 + \textrm{max}_i \{- v_i \} \}$ and the logistic loss $l(v) = \textrm(log)_2 (1 + \sum_i \textrm{exp} (- v_i))$ for $v \in R^k$. Then the supervised (sup) loss of the downstream task classifier $g$ is 
    $L_{sup}(\mathbf{T}, g) = E [l( \{g(x)_c - g(x)_{c'} \}_{c \neq c'})]$.
For simplicity, we use $L_{sup}(f)$ to denote the downstream loss of the model with function $f()$ which satisfies $L_{sup}(\mathbf{T}, g)$ and $g(x) = w f(x)$.
We outline the objective of contrastive learning: $k$ denotes number of negative samples used for training.
The unsurpervise loss can be defined as 
$L_{un}(f) = E[l(\{f(x)^T (f(x^+) - f(x^-)\}_{i=1}^k)]$.
After training, suppose $\hat{f}$ is the function which can minimizes the empirical unsupervised loss
and we denote its corresponding loss for supervised downstream task as $L_{sup}(\hat{f})$.
According to the theorem 4.1 in ~\cite{bound}, we have
\begin{align}\label{upper_bond}
    L_{sup}(\hat{f}) <= \alpha L_{un}(f) + \eta Gen_M + \epsilon
\end{align}
where $Gen$ is the generalization error which is defined as 
\begin{align}
Gen_M = O(R \sqrt{k} \frac{R_s (F)}{M} + (R^2 + log k) \sqrt{\frac{log \frac{1}{\epsilon}}{M}})
\end{align}
and $M$ is the sample size, $R_s (F)$ is the Rademacher average of $F$. 

\noindent{\bf C - Skip-connection Based Model.}
Suppose we use neural network with skip connection to learn the contrastive embedding, we have 
\begin{align*}
&L_{un}(f) = E[l(\{f_2(x)^T (f_2(x^+) - f_2(x^-)\}_{i=1}^k)] \\
 &= E[l(\{(f_I(x) + f_1(x))^T (f_I(x^+) + f_1(x^+) 
- f_I(x^-) - f_1(x^-)\}_{i=1}^k)] 
\end{align*}
where $l()$ is the logistic loss.
If we assume that the weights for $f_1(x)$ are also identity matrix $\mathrm{I}$ and $f_I(x)^T (f_I(x^+) - f_I(x^-)) >= 0$ which is a typical instance, we can have
\begin{align*}
L_{un}(f) &= E[l(4 \{f_I(x)^T (f_I(x^+) - f_I(x^-)\}_{i=1}^k)] \\
& <= E[l(\{f_I(x)^T (f_I(x^+) - f_I(x^-)\}_{i=1}^k)]
\end{align*}
which means the upper bond of skip connection is smaller than $f_I$.
When the weights for $f_1(x)$ are not identity matrix,
according to the universal approximation theory of deep neural network, 
$L_{un}(f)$ should be smaller or equal than $L_{un}(f_I)$.

The identity MLP, $f(x) = \mathbf{I} \mathbf{I} \mathbf{I} \mathbf{I} x = x$, is a special case of an MLP. 
Bring it to Eq.~\eqref{upper_bond}, 
This implies that the loss of a skip connection should not be greater than that of the identity MLP. Therefore, the upper bound for using skip connection for learning should be lower.



% For simplicity, we use $L_{sup}(f)$ to denote the supervised (sup) downstream loss of the model with function $f()$ which satisfies $L_{sup}(\mathbf{T}, g)$ and $g(x) = w f(x)$.
% After training, suppose $\hat{f}$ is the function which can minimizes the empirical unsupervised loss
% and we denote its corresponding loss for supervised downstream task as $L_{sup}(\hat{f})$.
% According to the theorim 4.1 in ~\cite{bound}, we have
% \begin{align}\label{upper_bond}
%     L_{sup}(\hat{f}) <= \alpha L_{un}(f) + \eta Gen_M + \epsilon
% \end{align}
% Substitue $\hat{f}$ with skip-connection based model and identity MLP respectively, it shows the loss of the skip-connection based model is not greater than that of the identity MLP. Therefore, the upper error bound for skip-connection based model should be not larger than the original upper error bound. See Appendix for more details.

We have observed that the proposed \myModel\ exhibits several similar properties to Adapter ~\cite{houlsby2019parameterefficient} in that both employ skip connection as their fundamental components as shown in Figure ~\ref{skip_connection}(d). However, Adapter is embedded within each layer of Transformer ~\cite{transformer}, while \myModel\ is positioned outside the original model $h()$. Although Adapter has been widely used in many Transformer ~\cite{transformer} based models ~\cite{bert, liu2019roberta}, no theoretical proof has been given thus far. In this work, we present the first theoretical proof demonstrating why skip connection-based refinement does not degrade downstream tasks. 

%We have observed that \myModel exhibits similar properties to Adapter ~\cite{...} in that both employ skip-connection as their funcdamental component. However, skip-connection in \myModel is positioned outside .... h(.) while in Adapter, the skip connection is embedded...... Despite .....



\begin{table*}
	\centering
	\caption{Compare with SimCSE on Different Downstream Tasks by Precision.}
	\vspace{-1\baselineskip}
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
	\hline
	Model         & eval\_CR & eval\_MPQA & eval\_MR  & eval\_MRPC  & eval\_SST2 & eval\_SUBJ & eval\_TREC \\ \hline
	%BERT & \cellcolor{lightgray} 81.35 & 81.88 & \cellcolor{lightgray}  74.36 & 69.33 & \cellcolor{lightgray} 79.13 & \cellcolor{lightgray} 93.02 & 67.08 \\  \hline
    %BERT + \myModel\ & 77.22 & 82.32 & 71.01 & 69.16 & 76.95 & 90.2  & \cellcolor{lightgray} 74.05 \\  \hline
    %BERT + \myModel\ (mask+noise) & 79.7  & \cellcolor{lightgray} 83.25 & 72.05 & \cellcolor{lightgray} 69.38 & 76.95 & 91.55 & 66.64 \\  \hline
    SimCSE & 85.99 & 88.5  & 80.54 & 73.65 & \textbf{86.47}  & 94.8  & \textbf{82.19}  \\  \hline
    SimCSE + \myModel\ & \textbf{86.36}   & 88.27 & \textbf{80.82}   & 74.71 & 85.55 & 94.93 & 80.8  \\  \hline
    SimCSE + \myModel\ (mask+gaussian) & 85.44 & \textbf{88.56}  & 78.25 & \textbf{75.01}  & 82.96 & \textbf{95.28}  & 80.1  \\  \hline
	
	\end{tabular}
	\label{simCSE_res}
	\vspace{-1\baselineskip}
\end{table*}


==> cikm/004_experiment.tex <==



This section assesses the performance of \myModel. Three base methods focusing on different scenarios are used which are FedE ~\cite{fedE} (federated learning), SimCLR ~\cite{simCLR} (unsupervised learning) and GraphSAGE ~\cite{graphsage} (supervised learning).
%\hh{merge sec 4.1 and 4.2 into a single subsection: Experimental Setting}
%The study utilizes five datasets, which are movieQA, STL10, CIFAR10, Cora and Pubmed. The details of each dataset can be found in Appendix.
%The following methods are employed to learn the input embedding for contrastive learning: FedE ~\cite{fedE}, SimCLR ~\cite{simCLR} and GraphSAGE ~\cite{graphsage}.
%The details of each baseline method can be found in Appendix. 

\subsection{Contrastive Learning for Federated Learning}
First, we evaluate \myModel\ for federated learning. To perform the evaluation, we randomly generate two knowledge graphs from the movieQA dataset ~\cite{tapaswi2016movieqa}. The entity embeddings are then learned using the fedE approach, as proposed by ~\cite{fedE}.
Three different downstream tasks are used in total. The first task involves providing a query movie and utilizing k-nearest neighbors (KNN) to identify the 10 closest movies in terms of their embedding distance. Subsequently, we determine the percentage of movies among these ten that share the same genre as the query movie.
The second task revolves around genre prediction, wherein we aim to predict the genre of a movie solely based on its embedding.
The third downstream task is movie recommendation which recommends new movies to users according to the user's watching history. The user history data is from Netflix dataset \footnote{https://www.kaggle.com/code/laowingkin/netflix-movie-recommendation/data}.
The results of different methods are shown in Table ~\ref{fede}. As we can see, using \myModel\ can actually improve the downstream task accuracy. For KNN task, the absolute improvement is about 4\%. For Genre prediction and movie recommendation, the average absolute improvement is 2\% and 0.2\%, respectively. 
\begin{table}[h]
	\centering
	\caption{Precision on different tasks for Federated Learning.}
	\vspace{-1\baselineskip}
	\begin{tabular}{|c|c|c|c|c|c|c|}
	\hline
	        & KNN & \makecell{ Genre \\ Prediction }  & \makecell{ Movie \\ Recommendation } \\ \hline
	FedE   & 58.51  & 84.83 &  7.47  \\ \hline
	\myModel + mask  & 62.83 & \textbf{86.12}   & \textbf{7.67} \\ \hline
        \myModel + gaussian  & \textbf{63.32} & 86.01   & 7.01 \\ \hline
	\end{tabular}
        \label{fede}
        \vspace{-1\baselineskip}
\end{table}

\subsection{Contrastive Learning for Image Classification}

Second, we test the performance of using contrastive learning to refine the embedding learned by unsupervised learning. Two datasets are used in this part which are STL10 and cifar10. We first use SimCLR ~\cite{simCLR} to learn the embedding for each image in the dataset, then we use the proposed model to relearn the embedding. The downstream task will predict the image class according to the image embedding. Table ~\ref{contrastive_task} shows the results. As we can see, using \myModel\ to further finetune the embedding space can improve the downstream task accuracy about 1\% in average. 
\begin{table}[h]
	\centering
	\caption{Precision on different dataset for Contrastive Learning.}
	\vspace{-1\baselineskip}
	\begin{tabular}{|c|c|c|c|c|c|c|}
	\hline
	   Image Classification     &  STL10 &  CIFAR10  \\ \hline
	SimCLR   & 76.09  & 66.88   \\ \hline
	\myModel + mask  & 75.84  &  65.93 \\ \hline
        \myModel + gaussian  & \textbf{77.73}   &  \textbf{67.02}  \\ \hline
	\end{tabular}
        \label{contrastive_task}
        \vspace{-1\baselineskip}
\end{table}

\subsection{Contrastive Learning for Supervised Learning}

Finally, we test the performance of using contrastive learning to refine the embedding learned by supervised learning. We use GraphSAGE ~\cite{graphsage} as the baseline methods. Two datasets are used in the experiments which are Cora and Pubmed. These two datasets are adopted from GraphSAGE. In the experiment, we first train GraphSAGE in supervised setting and treat the output of the second to last layer as the node embedding, then we use our proposed contrastive learning to refine the embedding. For the downstream task will predict the node label according to the node embedding.

We find that \myModel\ can further improve the downstream task performance. This exceeds our expectations as our initial hypothesis was that the embedding trained by supervised learning should fit the downstream task best, and further refinement of the embedding could decrease the downstream task performance. However, the experiment results show that skip connection contrastive learning method can further improve the downstream task performance.
\vspace{-0.5\baselineskip}
\begin{table}[h]
	\centering
	\caption{Precision on different dataset for Supervised Learning.}
	\vspace{-1\baselineskip}
	\begin{tabular}{|c|c|c|c|c|c|c|}
	\hline
	        & Cora & Pubmed  \\ \hline
	GraphSAGE   &  82.60 & 81.60   \\ \hline
	\myModel + mask  & 82.60  &  81.80 \\ \hline
        \myModel + gaussian  & \textbf{82.90}   &  \textbf{82.90}  \\ \hline
	\end{tabular}
        \label{contrastive_task}
        \vspace{-1\baselineskip}
\end{table}

\vspace{-0.5\baselineskip}
\subsection{Compare with SimCSE}
Another model, SimCSE ~\cite{gao2021simcse}, presents a similar idea to ours, however, they focus on language modeling. The authors propose a simple and efficient contrastive learning method for sentence embeddings. They pass the same input sentence through a pre-trained transformer-based language model, such as BERT ~\cite{bert}, twice with different dropout applied to obtain two different embeddings. These embedding pairs are then treated as positive examples for training. 
When learning the embedding for \myModel, we first freeze SimCSE, then use \myModel\ to refine the embedding. 
We evaluate these two models on the following tasks: CR ~\cite{CR}, MPQA ~\cite{MPQA}, MR ~\cite{MR}, MRPC ~\cite{MRPC}, SST-2 ~\cite{SST-2}, SUBJ ~\cite{SUBJ}, TREC ~\cite{TREC}. These 7 tasks are the same as ~\cite{gao2021simcse}. The results are shown in Table ~\ref{simCSE_res}. As we can see, the refined embedding  performs better on most downstream tasks. This indicates that the stacking of two refinement solutions is effective. Moreover, since \myModel\ operates in the embedding space, it enables easy integration of any desired data augmentation techniques.



==> cikm/005_related_work.tex <==



%\subsection{Representation Learning}

%The goal of representation learning is to learn low dimension vectors of the input data so that similar data will be close to each other in the embedding space, while dissimilar data will be far from each other. 
%For example, representation learning methods like TransE \cite{transE}, RESCAL ~\cite{RESCAL} and DistMult ~\cite{DistMult} embed entities in the konwledge graph as points in the low dimensional Euclidean and model relations as linear or bilinear transformation in the space.  Other methods like RotatE ~\cite{rotatE} and ComplEx ~\cite{complEx} represent entities as points in the complex space and relations as rotation or bilinear transfromation. Other methods like BoxE ~\cite{boxe} and KG2E ~\cite{gaussian_embedding} use geometry box or Gaussian distribution to represent an entity.


%\subsection{Contrastive Learning}

%Contrastive Learning focuses on minimizing the distance between the target embedding (anchor) vector and the matching (positive) embedding vector, while maximizing the distance between the anchor vector and the non-matching (negative) embedding vectors. Recent work on contrastive learning have shown that discriminative or contrastive approaches can (i) produce transferable embeddings for visual objects through the use of data augmentation ~\cite{simCLR}, and (ii) learn joint visual and language embedding space that can be used to perform zero-shot detection ~\cite{zero}. Given the sparseness and long-tailed property of scene graph datasets, application (i) of contrastive approach can help the model learn better visual appearance embeddings of (subject, object) pairs under limited resource settings. Moreover, in application (ii), contrastive learning gives a clearer separation of the visual embeddings and language embeddings compared to the traditional black-box neural fusion approaches ~\cite{resnet}, giving us more control over both the symbolic triples input and the final output embedding spaces.

%\subsection{Theoratical Proof}


%The goal of representation learning is to learn low dimension vectors of the input data so that similar data will be close to each other in the embedding space, while dissimilar data will be far from each other. 
%For example, representation learning methods like TransE \cite{transE}, RESCAL ~\cite{RESCAL} and DistMult ~\cite{DistMult} embed entities in the konwledge graph as points in the low dimensional Euclidean and model relations as linear or bilinear transformation in the space.  Other methods like RotatE ~\cite{rotatE} and ComplEx ~\cite{complEx} represent entities as points in the complex space and relations as rotation or bilinear transfromation. Other methods like BoxE ~\cite{boxe} and KG2E ~\cite{gaussian_embedding} use geometry box or Gaussian distribution to represent an entity.


==> cikm/006_conclusion.tex <==



In this paper, we propose a skip connection based contrastive learning framework (\myModel) which refine the input embedding space. We theoretically prove that the downstream task error uppper bounds will not be larger than original error upper bounds after
applying \myModel. The experiment results show the effectiveness of the proposed method. For future work, we intend to explore diverse data augmentation methods and continue reducing the error bound in theoretical analysis. Besides, we plan to analyze how \myModel\ and related architectures can address the issues raised in Figure ~\ref{problem_of_existing_method}. 





==> cikm/xxxx.tex <==
This section assesses the performance of \myModel. Three base methods focusing on different scenarios are used which are FedE ~\cite{fedE} (federated learning), SimCLR ~\cite{simCLR} (unsupervised learning) and GraphSAGE ~\cite{graphsage} (supervised learning).
The details of all datasets and base methods can be found in Appendix.
%\hh{merge sec 4.1 and 4.2 into a single subsection: Experimental Setting}
%The study utilizes five datasets, which are movieQA, STL10, CIFAR10, Cora and Pubmed. The details of each dataset can be found in Appendix.
%The following methods are employed to learn the input embedding for contrastive learning: FedE ~\cite{fedE}, SimCLR ~\cite{simCLR} and GraphSAGE ~\cite{graphsage}.
%The details of each baseline method can be found in Appendix. 


\subsection{Contrastive Learning for Federated Learning}

In this section, we evaluate \myModel\ forthe effectiveness of utilizing contrastive learning to enhance the embeddings obtained through federated learning. To perform the evaluation, we randomly generate two knowledge graphs from the movieQA dataset. The entity embeddings are then learned using the fedE approach, as proposed by ~\cite{fedE}.
Three different downstream tasks are used in total. The first task involves providing a query movie and utilizing k-nearest neighbors (knn) to identify the 10 closest movies in terms of their embedding distance. Subsequently, we determine the percentage of movies among these ten that share the same genre as the query movie.
The second task revolves around genre prediction, wherein we aim to predict the genre of a movie solely based on its embedding.
The third downstream task is movie recommendation which recommends new movies to users according to the user's watching history. The data is from Netflix dataset \footnote{https://www.kaggle.com/code/laowingkin/netflix-movie-recommendation/data}. More details can be found in Appendix.

The results of different methods are shown in Table ~\ref{fede}. As we can see, using \myModel\ can actually improve the downstream task accuracy. For KNN task, the improvement is about 4\%. For Genre prediction and movie recommendation, the average improvement is 2\% and 0.2\%, respectively. 

\begin{table}[h]
	\centering
	\caption{Precision on different tasks for Federated Learning.}
	\vspace{-1\baselineskip}
	\begin{tabular}{|c|c|c|c|c|c|c|}
	\hline
	        & KNN & \makecell{ Genre \\ Prediction }  & \makecell{ Movie \\ Recommendation } \\ \hline
	FedE   & 58.5  & 84.8 &  7.47  \\ \hline
	\myModel + mask  & 62.8 & \textbf{86.1}   & \textbf{7.67} \\ \hline
        \myModel + gaussian  & \textbf{63.3} & 86.0   & 7.01 \\ \hline
	\end{tabular}
        \label{fede}
        \vspace{-1\baselineskip}
\end{table}

\subsection{Contrastive Learning for Contrastive Learning}

In this section, we test the performance of using contrastive learning to refine the embedding learned by unsupervised learning. Two datasets are used in this part which are STL10 and cifar10. We first use SimCLR ~\cite{simCLR} to learn the embedding for each image in the dataset, then we use the proposed model to relearn the embedding. The downstream task will predict the image class according to the image embedding. Table ~\ref{contrastive_task} shows the results. As we can see, using \myModel\ to further finetune the embedding space can improve the downstream task accuracy about 1\% in average. 


\begin{table}[h]
	\centering
	\caption{Precision on different dataset for Contrastive Learning.}
	\vspace{-1\baselineskip}
	\begin{tabular}{|c|c|c|c|c|c|c|}
	\hline
	   Image Classification     &  STL10 &  CIFAR10  \\ \hline
	SimCLR   & 76.09  & 66.88   \\ \hline
	\myModel + mask  & 75.84  &  65.93 \\ \hline
        \myModel + gaussian  & \textbf{77.73}   &  \textbf{67.02}  \\ \hline
	\end{tabular}
        \label{contrastive_task}
        \vspace{-1\baselineskip}
\end{table}


\subsection{Contrastive Learning for Supervised Learning}

In this section, we test the performance of using contrastive learning to refine the embedding learned by supervised learning. We use GraphSAGE ~\cite{graphsage} as the baseline methods. Two datasets are used in the experiments which are Core and Pubmed. These two datasets are adopted from GraphSAGE. In the experiment, we first train GraphSAGE in supervised setting and treat the output of the second to last layer as the node embedding, then we use our proposed contrastive learning to refine the embedding. For the downstream task will , it is used to predict the node label according to the node embedding.

WAccording to the experiment results, we find that \myModel\ the skip connection contrastive learning method can further improve the downstream task performance. This is totally out of our expectation. Because we originally think that the embedding trained by supervised learning should fit the downstream task best, and further refinetune the embedding should decrease the downstream task performance. However, the experiment results show that skip connection contrastive learning method can further improve the downstream task performance.

\begin{table}[h]
	\centering
	\caption{Precision on different dataset for Supervised Learning.}
	\vspace{-1\baselineskip}
	\begin{tabular}{|c|c|c|c|c|c|c|}
	\hline
	        & Cora & Pubmed  \\ \hline
	GraphSAGE   &  82.60 & 81.6   \\ \hline
	\myModel + mask  & 82.60  &  81.8 \\ \hline
        \myModel + gaussian  & \textbf{82.90}   &  \textbf{82.9}  \\ \hline
	\end{tabular}
        \label{contrastive_task}
        \vspace{-1\baselineskip}
\end{table}


\subsection{Compare with SimCSE}

Another model, SimCSE ~\cite{gao2021simcse}, presents a similar idea to ours, however, they focus on language modeling. The authors propose a simple and efficient contrastive learning method for sentence embeddings. They pass the same input sentence through a pre-trained transformer-based language model, such as BERT ~\cite{bert}, twice with different dropout applied to obtain two different embeddings. These embedding pairs are then treated as positive examples for training. 
When learning the embedding for \myModel, we first fix SimCSE, then use \myModel\ to refine the embedding. 
We evaluate these two models on the following tasks: CR ~\cite{CR}, MPQA ~\cite{MPQA}, MR ~\cite{MR}, MRPC ~\cite{MRPC}, SST-2 ~\cite{SST-2}, SUBJ ~\cite{SUBJ}, TREC ~\cite{TREC}. These 7 tasks are the same as ~\cite{gao2021simcse}. The results are shown in Table ~\ref{simCSE_res}. As we can see, the refined embedding can performs better on most downstream tasks.


